Benchmarking Large Language Models for News Summarization

Large language models (LLMs) have shown promise for automatic summarization but the reasons behind their successes are poorly understood. By conducting a human evaluation on ten LLMs across different pretraining methods, prompts, and model scales, we make two important observations. First, we find instruction tuning, and not model size, is the key to the LLM's zero-shot summarization capability. Second, existing studies have been limited by low-quality references, leading to underestimates of human performance and lower few-shot and finetuning performance. To better evaluate LLMs, we perform human evaluation over high-quality summaries we collect from freelance writers. Despite major stylistic differences such as the amount of paraphrasing, we find that LMM summaries are judged to be on par with human written summaries.

==> sections/metrics_analysis.tex <==
\section{Evaluating Automatic Metrics}
\subsection{Experimental Setup}
\subsection{Experimental Results}

==> sections/related_work.tex <==
\section{Related Work}
Large-scale datasets \cite{cnndm,xsum,Rush_2015} along with more effective neural systems for conditional generation has lead to steady progress on abstractive summarization over the years \cite{Rush_2015,nallapati-etal-2016-abstractive,see-etal-2017-get,chen-bansal-2018-fast,dong2019unified}. The advent of pre-trained language models (PLMs) enabled a quantum leap in summarization capability, as current state-of-the-art (SOTA) summarization models produce remarkably fluent abstractive summaries by finetuning PLMs on existing summarization datasets \cite{liu-lapata-2019-text,bart,pegasus,brio}. Unlike most prior work in summarization that relies on large-scale datasets for training summarizers, our work explores zero-shot and few-shot summarization capability of LLMs and compares them to SOTA summarizer as well as human writers.

Most work in summarization has relied on automated reference-based evaluation \cite{Lin2004ROUGEAP,bert-score,Sellam2020BLEURTLR} in order to measure progress in summarization capability. Reference-based metrics, however, have been shown to have poor correlation with human judgements of summarization quality along key aspects such as faithfulness and relevance \cite{DBLP:conf/aaai/CaoWLL18,durmus-etal-2020-feqa,maynez-etal-2020-faithfulness,fabbri2020summeval,deutsch-roth-2021-understanding}. While the field has attempted to address these issues using reference-free evaluation metrics \cite{durmus-etal-2020-feqa,wang-etal-2020-asking,nan-etal-2021-improving,fabbri-etal-2022-qafacteval,kryscinski-etal-2020-evaluating,goyal-durrett-2020-evaluating,Laban2021SummaCRN}, recent work shows that these metrics are not robust and rely mostly on spurious measures \cite{durmus-etal-2022-spurious}. Our work shows that existing automated metrics are unable to reliably compare across different types of systems (finetuned vs. LLMs), though they do a reasonable job of distinguishing among the different LLM systems. Furthermore, our results show that improving the quality of existing references leads to improved performance of reference-based evaluation metrics, indicating that the ineffectiveness of reference-based evaluation in prior work may be overstated.

\citet{gpt3-era} is the work that's the closest to our study since they show that LLMs can produce remarkably good summaries in zero-shot settings, and outperform finetuned, SOTA systems according to humans. Their study only focuses on a single LLM, whereas in our work we evaluate ten different LLMs, and show that instruction tuning is the key to good summarization performance. We further collect human-written summaries, and show that the summaries generated by the best instruct-tuned LLM are on par with the huamn-written ones. 
